DNF: Unconditional 4D Generation with Dictionary-based Neural Fields

While remarkable success has been achieved through diffusion-based 3D generative models for shapes, 4D generative modeling remains challenging due to the complexity of object deformations over time. We propose DNF, a new 4D representation for unconditional generative modeling that efficiently models deformable shapes with disentangled shape and motion while capturing high-fidelity details in the deforming objects. To achieve this, we propose a dictionary learning approach to disentangle 4D motion from shape as neural fields. Both shape and motion are represented as learned latent spaces, where each deformable shape is represented by its shape and motion global latent codes, shape-specific coefficient vectors, and shared dictionary information. This captures both shape-specific detail and global shared information in the learned dictionary. Our dictionary-based representation well balances fidelity, contiguity and compression -- combined with a transformer-based diffusion model, our method is able to generate effective, high-fidelity 4D animations.

==> sections/experiment_3d.tex <==
\section{Experiments and Results}
\begin{table}[t]
\begin{center}
\resizebox{.95\columnwidth}{!}{
\begin{tabular}{c|c|c|c}
\hline
Method & MMD \downarrow & COV($\%$) \uparrow & 1-NNA($\%$) \downarrow \\ \hline
HyperDiffusion & 22.4 & 34.8 & 76.7 \\ 
Motion2vecsets & 18.7 & 48.1 & 68.2 \\ 
Ours & \textbf{17.5} & \textbf{54.1} & \textbf{58.2}  \\
\hline
\end{tabular}}

% \multicolumn{1}{|l|}{Category} & Method         & CD             \\ \hline
% \multirow{3}{*}{Plane}         & DeepSDF        & 0.063          \\ \cline{2-3} 
%                                & HyperDiffusion & \textbf{0.047} \\ \cline{2-3} 
%                                & Ours           & 0.050          \\ \hline
% \multirow{2}{*}{Animal}        & DeepSDF        & 0.055          \\ \cline{2-3} 
%                                & Ours           & \textbf{0.046} \\ \hline

\end{center}
\caption{Quantitative comparisons of 4D unconditional generation of animation sequences.}
\label{tab: rec}
\end{table}

\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.9\columnwidth]{figs/rec_qua.pdf}
\end{center}
   \caption{Qualitative comparisons for shape reconstruction with DeepSDF: (a) the ground truth mesh, (b) the reconstruction of DeepSDF, (c) our reconstruction after fine-tuning the coefficient vectors $\boldsymbol{\sigma}$, and (d) our reconstruction after the residual learning.}
   
\label{fig:rec_qua}
\end{figure}

\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.99\columnwidth]{figs/inter.pdf}
\end{center}
   \caption{Linear interpolations between two shapes in the weight space of (a) HyperDiffusion, (b) DeepSDF, and (c) our method}
   
\label{fig:inter}
\end{figure}

In this section, we first describe our experimental setup and the implementation details of our method. Second, we evaluate our proposed 3D representation in terms of quality and continuity. Finally, our generative model is evaluated from both a quality and novelty perspective. 

\subsection{Experiments Setup}
To evaluate the effectiveness of our method, we choose the airplane class of the ShapeNet dataset and the animal class in the DeformingThings4D dataset, which contains different types of animals, making it a more diverse training set.  Following prior works, we prepare the SDF samples by sampling 500,000 points around the object surface and uniformly in the unit sphere.  

In our experiment, we use 256 dimensional latent vectors and an 8-layer 512-dim MLP to learn a general view of the whole 3D class. Then we conduct SVD on the MLP parameters of each layer and fine-tune the coefficient vectors for 1000 epochs. 
For the airplane class, we learn the residual of batches of 8 samples with matrices of rank 3.  
For the animal class, which is relative easier but more diverse, we conduct residual learning for the first few samples of a species.
After representation learning, we use a list of 9 vectors, a latent vector and 8 coefficient vectors for each MLP layer, to represent a 3D shape.
The following diffusion model is trained for 6000 epochs in the weight space. We implement our models on the Pytorch framework \cite{paszke2017automatic} on NVIDIA 3090 GPUs.

\subsection{Shape Representation}
We evaluate our representation from two aspects: reconstruction quality and the contiguity of its weight space, and show output meshes extracted with Marching Cubes.
As shown in the Table \ref{tab: rec}, our method outperforms DeepSDF by a large margin in terms of Chamfer Distance (CD) in both plane class and animal class, and gets comparable results with HyperDiffusion on plane class, which optimizes a MLP for every shape in the class, at the cost of discontinuity of their weight space. 

Additionally, we compare our reconstruction to DeepSDF qualitatively. As shown in the Figure \ref{fig:rec_qua}, our reconstructions have better quality than DeepSDF, and display finer details at the local level.

We evaluate the contiguity of the representations by linear interpolation in their weight space. We present an example in Figure \ref{fig:inter} to show the comparisons between different representations. 
HyperDiffusion represents 3D shapes as MLP weights without shared structures in their weight space, resulting in meaningless interpolations. As deepSDF represents shapes as a single global vector, it does not present good local details, and its interpolations also suffer from low-quality. In contrast, we represent shapes as global latent plus coefficient vectors, which allows for precise and reliable interpolation. 

\subsection{Unconditional shape generation}
We compare our methods with other 3D shape generation methods and some variants of ours in terms of both quality and novelty.

\textbf{Shape Quality.} To evaluate the generation quality, we follow the previous works and choose (i) Minimum Matching Distance (MMD), measuring the fidelity of the generated shapes; (ii) coverage (COV) indicating how well the generated shapes cover the shapes in the given 3D training set; (iii) 1-NN classifier accuracy (1-NNA) measuring how well a classifier differentiates the generated shapes from those in the training set and (iv) Frechet Pointnet++ Distance (FPD) measures the distance of two distributions via features extracted by a 3D Pointnet++ network \cite{qi2017pointnet++}, analogous to the commonly used Frechet Inception Distance (FID score) \cite{heusel2017gans} in the 2D domain. 


\begin{table}[t]
\begin{center}
\resizebox{.99\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{Category} & Method         & MMD $\downarrow$ & COV(\%) $\uparrow$ & 1-NNA(\%) $\downarrow$ & FPD $\downarrow$ \\ \hline
\multirow{4}{*}{Plane}         & HyperDiffusion & 3.6          & 48.8          & \textbf{68.5} & \textbf{4.23} \\ \cline{2-6} 
                               & DeepSDF         & 3.7 & 32.7    & 7.2       & 9.39 \\ \cline{2-6} 
                               & Ours           & 3.4 & 44.4    & 69.2      & 4.28 \\ \cline{2-6} 
                               & Ours$_{inter}$    & \textbf{3.2} & \textbf{49.7}    & 72.2      & 4.42 \\ \hline
\multirow{2}{*}{Animal}        & Ours           & \textbf{6.4} & \textbf{54.7} & \textbf{60.0} & \textbf{1.69} \\ \cline{2-6} 
                               & Ours$_{inter}$     & 6.9 & 47.9    & 65.2      & 2.97 \\ \hline
\end{tabular}}
\end{center}
\caption{Quantitative comparison on unconditional 3D shape generation for the plane and animal categories. Our method outperforms other methods in terms of MMD and COV and gets comparable results in 1-NNA and FPD with HyperDiffusion.}
\label{tab: gen_quan}
\end{table}

\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.99\columnwidth]{figs/gen_qua.pdf}
\end{center}
   \caption{Visual comparisons with HyperDiffusion. Our generated shapes exhibit better stability and cleaner surfaces.  }
   
\label{fig:gen_qua}
\end{figure}

For the baselines, apart from HyperDiffusion, we also train a diffusion model on the latent vectors extracted by DeepSDF to generate new samples.
In order to encourage the diffusion model to generate more new shapes and alleviate the overfitting problem, we augment the training data with random interpolations and we denote this variant by the suffix \textit{inter}. 
As shown in Table \ref{tab: gen_quan}, for the plane class, our method outperforms other methods in terms of MMD and COV and gets comparable results in 1-NNA and FPD with HyperDiffusion. However, the performance degrades when adding interpolations during training in the animal class, which is more diverse and interpolations between different species may be unreliable and affect the generative performance. We also show some qualitative results of HyperDiffusion and our method in Figure \ref{fig:gen_qua}. HyperDiffusion is capable of generating samples with more delicate local details but also has a certain possibility to generate failure cases, while our method is more stable and can generate more cleaner surface without obvious artifacts. 

\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.95\columnwidth]{figs/novel2.pdf}
\end{center}
   \caption{Novel generated shapes and the nearest neighbor retrieval. For generated shapes (left) from our method, we look up the top-2 nearest neighbors (right) from the training set based on the Chamfer Distance. Our method can fuse features from known samples to generate new samples.}
\label{fig:novle}
\end{figure}


\begin{figure}[t]
\begin{center}
   \includegraphics[width=0.95\columnwidth]{figs/novelty.pdf}
\end{center}
   \caption{Distribution of LFDs for all generations with their nearest neighbors in plane class, showing that our method is able to generate sizeable novel shapes.}
   
\label{fig:novlety}
\end{figure}


\textbf{Shape novelty.} Next, we analyze whether our method can generate novel shapes, meaning that it does not simply memorize the training data. To do this, we generate 600 random shapes and retrieve its top-two nearest neighbors in the training set via Chamfer Distance and Light Field Distance (LFD), which is computed based on rendered images from multiple views and focuses more on visual similarity. 

First, we show some novel samples and their top-two nearest neighbors in Figure \ref{fig:novle} to demonstrate that our method is capable of fusing features from known samples to generate new samples.
We then plot the distribution of LFDs for all generated shapes in Figure \ref{fig:novlety}. As illustrated in the picture, most of our generations have similar shapes to their nearest neighbors but have differences in details. There also exists a sizable number of samples with LFDs greater than 5000, which means that they are brand new samples. Our method significantly reduces the overfitting problem in the generative model and can yield novel and reliable samples, which cannot be achieved with HyperDiffusion.  


\textbf{Analysis.}
Our method performs slightly worse than HyperDiffusion in terms of generation quality in FPD and we analyze the possible reasons. HyperDiffusion optimizes an independent MLP for each shape in a 3D class, representing shapes with very fine details at the cost the discontinuity of its weight space. In contrast, developed from DeepSDF, our method only fine-tunes a part of the global MLP parameters based on a single latent vector, which improves the representation ability but still limited compared to fine-tuning the whole MLP parameters. However, our representation preserves the underlying contiguity using this partial fine-tuning strategy, enabling the diffusion models to generate more novel and reliable shapes than HyperDiffusion.  


